NuSTAR and Suzaku observations of the hard state in Cygnus X-1: locating the inner accretion disk

We present simultaneous Nuclear Spectroscopic Telescope Array (NuSTAR ) and Suzaku observations of the X-ray binary Cygnus X-1 in the hard state. This is the first time this state has been observed in Cyg X-1 with NuSTAR, which enables us to study the reflection and broad-band spectra in unprecedented detail. We confirm that the iron line cannot be fit with a combination of narrow lines and absorption features, and instead requires a relativistically blurred profile in combination with a narrow line and absorption from the companion wind. We use the reflection models of Garcia et al. (2014) to simultaneously measure the black hole spin, disk inner radius, and coronal height in a self-consistent manner. Detailed fits to the iron line profile indicate a high level of relativistic blurring, indicative of reflection from the inner accretion disk. We find a high spin, a small inner disk radius, and a low source height, and rule out truncation to greater than three gravitational radii at the 3{\sigma} confidence level. In addition, we find that the line profile has not changed greatly in the switch from soft to hard states, and that the differences are consistent with changes in the underlying reflection spectrum rather than the relativistic blurring. We find that the blurring parameters are consistent when fitting either just the iron line or the entire broad-band spectrum, which is well modelled with a Comptonized continuum plus reflection model.

==> journal_defs.tex <==
\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup} 
\def\aj{AJ}%          % Astronomical Journal
\def\araa{ARA\&A}%          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%          % Astrophysical Journal
\def\apjl{ApJ}%          % Astrophysical Journal, Letters
\def\apjs{ApJS}%          % Astrophysical Journal, Supplement
\def\apss{Ap\&SS}%          % Astrophysics and Space Science
\def\aap{A\&A}%          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%          % Astronomy and Astrophysics, Supplement
\def\caa{Chinese Astron. Astrophys.}%          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%          % Chinese Journal of Astronomy and Astrophysics
\def\mnras{MNRAS}%          % Monthly Notices of the RAS
\def\na{New A}%          % New Astronomy
\def\nar{New A Rev.}%          % New Astronomy Review
\def\pasa{PASA}%          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%          % Physical Review C
\def\prd{Phys.~Rev.~D}%          % Physical Review D
\def\pre{Phys.~Rev.~E}%          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%          % Physical Review Letters
\def\pasp{PASP}%          % Publications of the ASP
\def\pasj{PASJ}%          % Publications of the ASJ
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%          % Revista Mexicana de Astronomia y Astrofisica
\def\ssr{Space~Sci.~Rev.}%                Space Science Reviews
\def\nat{Nature}%          % Nature
\def\iaucirc{IAU~Circ.}%          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%          % Astrophysics Letters
\def\procspie{Proc.~SPIE}%          % Proceedings of the SPIE


